Neighboring Words Affect Human Interpretation of Saliency Explanations

Word-level saliency explanations ("heat maps over words") are often used to communicate feature-attribution in text-based models. Recent studies found that superficial factors such as word length can distort human interpretation of the communicated saliency scores. We conduct a user study to investigate how the marking of a word's neighboring words affect the explainee's perception of the word's importance in the context of a saliency explanation. We find that neighboring words have significant effects on the word's importance rating. Concretely, we identify that the influence changes based on neighboring direction (left vs. right) and a-priori linguistic and computational measures of phrases and collocations (vs. unrelated neighboring words). Our results question whether text-based saliency explanations should be continued to be communicated at word level, and inform future research on alternative saliency explanation methods.

==> figures/shap_results/tables/phi_sq_875/importance_rating_model_anova_parametric.tex <==
% latex table generated in R 4.2.2 by xtable 1.8-4 package
% Thu Mar 23 09:36:25 2023
\begin{table}[ht]
\centering
\begin{tabular}{rrrr}
  \hline
 & df & F & p-value \\ 
  \hline
capitalization & 2.00 & 0.35 & 0.71 \\ 
  dependency\_relation & 35.00 & 3.47 & 0.00 \\ 
   \hline
\end{tabular}
\caption{Parametric terms.} 
\label{importance_rating_model_anova_parametric}
\end{table}


==> figures/shap_results/tables/phi_sq_875/importance_rating_model_anova_smooth.tex <==
% latex table generated in R 4.2.2 by xtable 1.8-4 package
% Thu Mar 23 09:36:25 2023
\begin{table}[ht]
\centering
\begin{tabular}{rrrrr}
  \hline
 & edf & Ref.df & F & p-value \\ 
  \hline
  s(saliency) & 6.71 & 19.00 & 18.85 & 0.00 \\ 
  s(display\_index) & 1.88 & 9.00 & 6.45 & 0.00 \\ 
  s(word\_length) & 2.04 & 9.00 & 4.43 & 0.00 \\ 
  s(sentence\_length) & 0.00 & 4.00 & 0.00 & 0.98 \\ 
  s(relative\_word\_frequency) & 0.00 & 9.00 & 0.00 & 0.64 \\ 
  s(normalized\_saliency\_rank) & 0.89 & 9.00 & 1.99 & 0.00 \\ 
  s(word\_position) & 0.42 & 9.00 & 0.12 & 0.19 \\ 
  te(left\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_leftFALSE & 0.00 & 24.00 & 0.00 & 0.37 \\ 
  te(left\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_leftTRUE & 0.00 & 24.00 & 0.00 & 0.49 \\ 
  te(right\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_rightFALSE & 0.99 & 24.00 & 0.20 & 0.06 \\ 
  te(right\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_rightTRUE & 3.24 & 24.00 & 1.09 & 0.01 \\ 
  s(sentence\_id) & 0.00 & 149.00 & 0.00 & 0.52 \\ 
  s(saliency,sentence\_id) & 11.31 & 150.00 & 0.10 & 0.14 \\ 
  s(worker\_id) & 34.77 & 35.00 & 14185.28 & 0.00 \\ 
  s(saliency,worker\_id) & 34.59 & 36.00 & 8468.22 & 0.00 \\ 
   \hline
\end{tabular}
\caption{Smooth terms.} 
\label{importance_rating_model_anova_smooth}
\end{table}


==> figures/shap_results/tables/phi_sq_875/importance_rating_model_params.tex <==
% latex table generated in R 4.2.2 by xtable 1.8-4 package
% Thu Mar 23 09:36:34 2023
\begin{table}[ht]
\centering
\begin{tabular}{lrrrr}
   \hline
A. parametric coefficients & Estimate & Std. Error & t-value & p-value \\ 
  (Intercept) & 3.2852 & 0.7487 & 4.3881 & $<$ 0.0001 \\ 
  capitalizationall\_upper & 0.1879 & 0.2481 & 0.7575 & 0.4488 \\ 
  capitalizationfirst\_upper & -0.0206 & 0.0875 & -0.2353 & 0.8140 \\ 
  dependency\_relationacl & 1.2511 & 0.2411 & 5.1887 & $<$ 0.0001 \\ 
  dependency\_relationacl:relcl & 1.6585 & 0.4057 & 4.0879 & $<$ 0.0001 \\ 
  dependency\_relationadvcl & 1.2577 & 0.3203 & 3.9271 & 0.0001 \\ 
  dependency\_relationadvmod & 1.1961 & 0.2386 & 5.0121 & $<$ 0.0001 \\ 
  dependency\_relationamod & 1.1070 & 0.1763 & 6.2797 & $<$ 0.0001 \\ 
  dependency\_relationappos & 1.2048 & 0.2490 & 4.8390 & $<$ 0.0001 \\ 
  dependency\_relationaux & 0.8742 & 0.3213 & 2.7213 & 0.0065 \\ 
  dependency\_relationaux:pass & 0.9116 & 0.2342 & 3.8923 & 0.0001 \\ 
  dependency\_relationcase & 0.7674 & 0.1382 & 5.5524 & $<$ 0.0001 \\ 
  dependency\_relationcc & 0.6231 & 0.2251 & 2.7681 & 0.0057 \\ 
  dependency\_relationccomp & 1.6839 & 0.5906 & 2.8511 & 0.0044 \\ 
  dependency\_relationcompound & 1.2727 & 0.1751 & 7.2685 & $<$ 0.0001 \\ 
  dependency\_relationcompound:prt & 0.9051 & 1.2073 & 0.7497 & 0.4535 \\ 
  dependency\_relationconj & 1.2347 & 0.2571 & 4.8024 & $<$ 0.0001 \\ 
  dependency\_relationcop & 0.7111 & 0.1891 & 3.7608 & 0.0002 \\ 
  dependency\_relationdep & 1.2656 & 0.8853 & 1.4295 & 0.1529 \\ 
  dependency\_relationdet & 0.7052 & 0.1446 & 4.8765 & $<$ 0.0001 \\ 
  dependency\_relationdet:predet & 2.0391 & 0.7693 & 2.6505 & 0.0081 \\ 
  dependency\_relationfixed & 1.8025 & 0.5309 & 3.3951 & 0.0007 \\ 
  dependency\_relationflat & 1.0599 & 0.2024 & 5.2381 & $<$ 0.0001 \\ 
  dependency\_relationmark & 1.0450 & 0.2950 & 3.5423 & 0.0004 \\ 
  dependency\_relationnmod & 1.4404 & 0.1916 & 7.5170 & $<$ 0.0001 \\ 
  dependency\_relationnmod:poss & 1.0869 & 0.3069 & 3.5417 & 0.0004 \\ 
  dependency\_relationnmod:tmod & 1.6254 & 0.2419 & 6.7181 & $<$ 0.0001 \\ 
  dependency\_relationnsubj & 1.1227 & 0.2034 & 5.5192 & $<$ 0.0001 \\ 
  dependency\_relationnsubj:pass & 1.5851 & 0.3234 & 4.9013 & $<$ 0.0001 \\ 
  dependency\_relationnummod & 1.3571 & 0.2923 & 4.6435 & $<$ 0.0001 \\ 
  dependency\_relationobj & 1.3917 & 0.2101 & 6.6246 & $<$ 0.0001 \\ 
  dependency\_relationobl & 1.3470 & 0.1736 & 7.7571 & $<$ 0.0001 \\ 
  dependency\_relationobl:agent & 1.9797 & 0.4554 & 4.3472 & $<$ 0.0001 \\ 
  dependency\_relationobl:npmod & 1.0808 & 0.6725 & 1.6071 & 0.1081 \\ 
  dependency\_relationobl:tmod & 1.4910 & 0.2569 & 5.8044 & $<$ 0.0001 \\ 
  dependency\_relationparataxis & 3.5373 & 1.3453 & 2.6294 & 0.0086 \\ 
  dependency\_relationroot & 1.3905 & 0.1856 & 7.4928 & $<$ 0.0001 \\ 
  dependency\_relationxcomp & 1.3159 & 0.4267 & 3.0843 & 0.0021 \\ 
   \hline
B. smooth terms & edf & Ref.df & F-value & p-value \\ 
  s(saliency) & 6.7099 & 19.0000 & 18.8480 & $<$ 0.0001 \\ 
  s(display\_index) & 1.8807 & 9.0000 & 6.4497 & $<$ 0.0001 \\ 
  s(word\_length) & 2.0427 & 9.0000 & 4.4298 & 0.0001 \\ 
  s(sentence\_length) & 0.0002 & 4.0000 & 0.0000 & 0.9831 \\ 
  s(relative\_word\_frequency) & 0.0003 & 9.0000 & 0.0000 & 0.6433 \\ 
  s(normalized\_saliency\_rank) & 0.8890 & 9.0000 & 1.9875 & 0.0023 \\ 
  s(word\_position) & 0.4209 & 9.0000 & 0.1191 & 0.1880 \\ 
  te(left\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_leftFALSE & 0.0025 & 24.0000 & 0.0001 & 0.3672 \\ 
  te(left\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_leftTRUE & 0.0007 & 24.0000 & 0.0000 & 0.4873 \\ 
  te(right\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_rightFALSE & 0.9899 & 24.0000 & 0.2022 & 0.0625 \\ 
  te(right\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_rightTRUE & 3.2375 & 24.0000 & 1.0908 & 0.0051 \\ 
  s(sentence\_id) & 0.0036 & 149.0000 & 0.0000 & 0.5228 \\ 
  s(saliency,sentence\_id) & 11.3094 & 150.0000 & 0.1009 & 0.1393 \\ 
  s(worker\_id) & 34.7690 & 35.0000 & 14185.2844 & $<$ 0.0001 \\ 
  s(saliency,worker\_id) & 34.5851 & 36.0000 & 8468.2186 & $<$ 0.0001 \\ 
   \hline
\end{tabular}
\caption{Smooth and parametric terms.} 
\label{importance_rating_model_params}
\end{table}


==> figures/shap_results/tables/phi_sq_875/word_pairs_left_lexical_chunks.tex <==
% latex table generated in R 4.2.2 by xtable 1.8-4 package
% Thu Mar 23 09:35:18 2023
\begin{table}[ht]
\centering
\begin{tabular}{rll}
  \hline
 & left\_word & word \\ 
  \hline
3768 & United & Kingdom \\ 
  2845 & All-Africa & Games \\ 
  2289 & Blyth & Spartans \\ 
  138 & Major & League \\ 
  853 & Milwaukee & Brewers \\ 
  199 & Rock & band \\ 
  343 & cassette & tape \\ 
  3050 & Arborophila & charltonii \\ 
  2449 & \& & B \\ 
  1135 & Special & Scientific \\ 
  1463 & Minor & Counties \\ 
  2420 & Julius & Caesar \\ 
  2075 & south & Wales \\ 
  63 & New & Zealand \\ 
  3080 & women & 's \\ 
   \hline
\end{tabular}
\caption{Word pairs that are lexical chunks following our definition (left neighbors).} 
\label{tab:word_pairs_left_lexical_chunks}
\end{table}


==> figures/shap_results/tables/phi_sq_875/word_pairs_left_no_lexical_chunks.tex <==
% latex table generated in R 4.2.2 by xtable 1.8-4 package
% Thu Mar 23 09:35:18 2023
\begin{table}[ht]
\centering
\begin{tabular}{rll}
  \hline
 & left\_word & word \\ 
  \hline
496 & In & December \\ 
  1324 & is & open \\ 
  4177 & Sorel & succeeded \\ 
  4699 & time & , \\ 
  282 & has & qualified \\ 
  2858 & The & ORC-International \\ 
  4119 & , & 2008 \\ 
  1437 & article & show \\ 
  4544 & begin & selling \\ 
  690 & was & remade \\ 
  1037 & Linkabit & was \\ 
  808 & businessman & and \\ 
  4521 & February & 2017 \\ 
  1599 & of & Industrial \\ 
  167 & , & it \\ 
   \hline
\end{tabular}
\caption{Word pairs that are no lexical chunks following our definition (left neighbors).} 
\label{tab:word_pairs_left_no_lexical_chunks}
\end{table}


==> figures/shap_results/tables/phi_sq_875/word_pairs_right_lexical_chunks.tex <==
% latex table generated in R 4.2.2 by xtable 1.8-4 package
% Thu Mar 23 09:35:18 2023
\begin{table}[ht]
\centering
\begin{tabular}{rll}
  \hline
 & word & right\_word \\ 
  \hline
4944 & secondary & school \\ 
  3880 & bass & guitar \\ 
  2905 & St & Mirren \\ 
  90 & Patria & Music/Theater \\ 
  888 & peer-reviewed & scientific \\ 
  174 & a & former \\ 
  319 & R & \& \\ 
  3548 & Val & Trompia \\ 
  1045 & Milwaukee & Brewers \\ 
  1278 & women & 's \\ 
  3517 & such & as \\ 
  2183 & football & team \\ 
  57 & home & games \\ 
  3845 & railway & station \\ 
  1574 & Blyth & Spartans \\ 
   \hline
\end{tabular}
\caption{Word pairs that are lexical chunks following our definition (right neighbors).} 
\label{tab:word_pairs_right_lexical_chunks}
\end{table}


==> figures/shap_results/tables/phi_sq_875/word_pairs_right_no_lexical_chunks.tex <==
% latex table generated in R 4.2.2 by xtable 1.8-4 package
% Thu Mar 23 09:35:18 2023
\begin{table}[ht]
\centering
\begin{tabular}{rll}
  \hline
 & word & right\_word \\ 
  \hline
4126 & coach & and \\ 
  4662 & it & would \\ 
  291 & entertainment & reporter \\ 
  2801 & on & 15 \\ 
  4089 & credited & for \\ 
  1468 & a & major \\ 
  4468 & the & constellation \\ 
  726 & level & . \\ 
  1078 & students & to \\ 
  835 & born & 22 \\ 
  4450 & in & Algeria \\ 
  1624 & on & E4 \\ 
  178 & from & 1997 \\ 
  51 & ( & ORCi \\ 
  302 & Skip & '' \\ 
   \hline
\end{tabular}
\caption{Word pairs that are no lexical chunks following our definition (right neighbors).} 
\label{tab:word_pairs_right_no_lexical_chunks}
\end{table}


==> tables/jaccard_875/importance_rating_model_anova_parametric.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 14:19:54 2023
\begin{table}[ht]
\centering
\begin{tabular}{rrrr}
  \hline
 & df & F & p-value \\ 
  \hline
capitalization & 2.00 & 3.11 & 0.04 \\ 
  dependency\_relation & 35.00 & 2.94 & 0.00 \\ 
   \hline
\end{tabular}
\caption{Parametric terms.} 
\label{importance_rating_model_anova_parametric}
\end{table}


==> tables/jaccard_875/importance_rating_model_anova_smooth.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 14:19:54 2023
\begin{table}[ht]
\centering
\begin{tabular}{rrrrr}
  \hline
 & edf & Ref.df & F & p-value \\ 
  \hline
s(saliency) & 11.19 & 19.00 & 569.26 & 0.00 \\ 
  s(display\_index) & 3.07 & 9.00 & 21.63 & 0.00 \\ 
  s(word\_length) & 1.61 & 9.00 & 16.51 & 0.00 \\ 
  s(sentence\_length) & 0.00 & 4.00 & 0.00 & 0.44 \\ 
  s(relative\_word\_frequency) & 0.00 & 9.00 & 0.00 & 0.85 \\ 
  s(normalized\_saliency\_rank) & 0.58 & 9.00 & 0.34 & 0.12 \\ 
  s(word\_position) & 0.60 & 9.00 & 0.18 & 0.17 \\ 
  te(left\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_leftFALSE & 3.09 & 24.00 & 1.45 & 0.00 \\ 
  te(left\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_leftTRUE & 0.75 & 24.00 & 0.06 & 0.27 \\ 
  te(right\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_rightFALSE & 2.66 & 24.00 & 0.65 & 0.02 \\ 
  te(right\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_rightTRUE & 1.04 & 24.00 & 0.12 & 0.18 \\ 
  s(sentence\_id) & 0.00 & 149.00 & 0.00 & 0.62 \\ 
  s(saliency,sentence\_id) & 16.45 & 150.00 & 0.14 & 0.18 \\ 
  s(worker\_id) & 62.19 & 63.00 & 30026.13 & 0.00 \\ 
  s(saliency,worker\_id) & 62.11 & 64.00 & 16856.17 & 0.00 \\ 
   \hline
\end{tabular}
\caption{Smooth terms.} 
\label{importance_rating_model_anova_smooth}
\end{table}


==> tables/jaccard_875/importance_rating_model_params.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 14:20:05 2023
\begin{table}[ht]
\centering
\begin{tabular}{lrrrr}
   \hline
A. parametric coefficients & Estimate & Std. Error & t-value & p-value \\ 
  (Intercept) & 5.0399 & 0.5456 & 9.2381 & $<$ 0.0001 \\ 
  capitalizationall\_upper & 0.2462 & 0.1691 & 1.4561 & 0.1454 \\ 
  capitalizationfirst\_upper & 0.1461 & 0.0651 & 2.2430 & 0.0249 \\ 
  dependency\_relationacl & 0.6221 & 0.1707 & 3.6443 & 0.0003 \\ 
  dependency\_relationacl:relcl & 1.0747 & 0.2896 & 3.7107 & 0.0002 \\ 
  dependency\_relationadvcl & 0.9879 & 0.2163 & 4.5675 & $<$ 0.0001 \\ 
  dependency\_relationadvmod & 0.2410 & 0.1732 & 1.3913 & 0.1642 \\ 
  dependency\_relationamod & 0.6780 & 0.1296 & 5.2306 & $<$ 0.0001 \\ 
  dependency\_relationappos & 0.5584 & 0.1867 & 2.9911 & 0.0028 \\ 
  dependency\_relationaux & -0.0281 & 0.2509 & -0.1121 & 0.9107 \\ 
  dependency\_relationaux:pass & 0.4614 & 0.1675 & 2.7548 & 0.0059 \\ 
  dependency\_relationcase & 0.2969 & 0.0989 & 3.0028 & 0.0027 \\ 
  dependency\_relationcc & 0.0015 & 0.1736 & 0.0087 & 0.9930 \\ 
  dependency\_relationccomp & 0.4917 & 0.4680 & 1.0507 & 0.2934 \\ 
  dependency\_relationcompound & 0.6047 & 0.1241 & 4.8741 & $<$ 0.0001 \\ 
  dependency\_relationcompound:prt & 0.4366 & 0.5597 & 0.7800 & 0.4354 \\ 
  dependency\_relationconj & 0.5452 & 0.1675 & 3.2558 & 0.0011 \\ 
  dependency\_relationcop & 0.1817 & 0.1429 & 1.2712 & 0.2037 \\ 
  dependency\_relationdep & 1.3444 & 1.0647 & 1.2627 & 0.2067 \\ 
  dependency\_relationdet & 0.0766 & 0.1065 & 0.7194 & 0.4719 \\ 
  dependency\_relationdet:predet & 1.2639 & 0.7235 & 1.7468 & 0.0807 \\ 
  dependency\_relationfixed & -0.0571 & 0.4250 & -0.1343 & 0.8932 \\ 
  dependency\_relationflat & 0.6416 & 0.1498 & 4.2823 & $<$ 0.0001 \\ 
  dependency\_relationmark & 0.1135 & 0.2151 & 0.5279 & 0.5976 \\ 
  dependency\_relationnmod & 0.8158 & 0.1366 & 5.9715 & $<$ 0.0001 \\ 
  dependency\_relationnmod:poss & 0.6841 & 0.2106 & 3.2489 & 0.0012 \\ 
  dependency\_relationnmod:tmod & 0.7570 & 0.1738 & 4.3556 & $<$ 0.0001 \\ 
  dependency\_relationnsubj & 0.4957 & 0.1515 & 3.2710 & 0.0011 \\ 
  dependency\_relationnsubj:pass & 0.3859 & 0.2158 & 1.7882 & 0.0738 \\ 
  dependency\_relationnummod & 0.7822 & 0.2377 & 3.2900 & 0.0010 \\ 
  dependency\_relationobj & 0.6429 & 0.1513 & 4.2498 & $<$ 0.0001 \\ 
  dependency\_relationobl & 0.7717 & 0.1271 & 6.0720 & $<$ 0.0001 \\ 
  dependency\_relationobl:agent & 0.6044 & 0.3574 & 1.6909 & 0.0909 \\ 
  dependency\_relationobl:npmod & 0.3661 & 0.8047 & 0.4549 & 0.6492 \\ 
  dependency\_relationobl:tmod & 0.7750 & 0.2089 & 3.7106 & 0.0002 \\ 
  dependency\_relationparataxis & 0.9420 & 0.8508 & 1.1071 & 0.2683 \\ 
  dependency\_relationroot & 0.6801 & 0.1314 & 5.1769 & $<$ 0.0001 \\ 
  dependency\_relationxcomp & 0.6792 & 0.2657 & 2.5567 & 0.0106 \\ 
   \hline
B. smooth terms & edf & Ref.df & F-value & p-value \\ 
  s(saliency) & 11.1937 & 19.0000 & 569.2584 & $<$ 0.0001 \\ 
  s(display\_index) & 3.0656 & 9.0000 & 21.6287 & $<$ 0.0001 \\ 
  s(word\_length) & 1.6051 & 9.0000 & 16.5092 & $<$ 0.0001 \\ 
  s(sentence\_length) & 0.0006 & 4.0000 & 0.0001 & 0.4408 \\ 
  s(relative\_word\_frequency) & 0.0006 & 9.0000 & 0.0000 & 0.8498 \\ 
  s(normalized\_saliency\_rank) & 0.5778 & 9.0000 & 0.3409 & 0.1205 \\ 
  s(word\_position) & 0.5997 & 9.0000 & 0.1848 & 0.1746 \\ 
  te(left\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_leftFALSE & 3.0917 & 24.0000 & 1.4517 & 0.0025 \\ 
  te(left\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_leftTRUE & 0.7466 & 24.0000 & 0.0572 & 0.2695 \\ 
  te(right\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_rightFALSE & 2.6619 & 24.0000 & 0.6461 & 0.0229 \\ 
  te(right\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_rightTRUE & 1.0358 & 24.0000 & 0.1199 & 0.1813 \\ 
  s(sentence\_id) & 0.0021 & 149.0000 & 0.0000 & 0.6187 \\ 
  s(saliency,sentence\_id) & 16.4541 & 150.0000 & 0.1397 & 0.1835 \\ 
  s(worker\_id) & 62.1894 & 63.0000 & 30026.1302 & $<$ 0.0001 \\ 
  s(saliency,worker\_id) & 62.1077 & 64.0000 & 16856.1655 & $<$ 0.0001 \\ 
   \hline
\end{tabular}
\caption{Smooth and parametric terms.} 
\label{importance_rating_model_params}
\end{table}


==> tables/jaccard_875/word_pairs_left_lexical_chunks.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 14:18:01 2023
\begin{table}[ht]
\centering
\begin{tabular}{rll}
  \hline
 & left\_word & word \\ 
  \hline
5332 & secondary & school \\ 
  4163 & scientific & journal \\ 
  3349 & south & Wales \\ 
  137 & guest & appearance \\ 
  910 & five & years \\ 
  150 & radio & station \\ 
  304 & fairy & tale \\ 
  4804 & elliptical & galaxy \\ 
  3819 & most & recent \\ 
  1220 & Blyth & Spartans \\ 
  1716 & New & Zealand \\ 
  3719 & backing & vocals \\ 
  3063 & Scientific & Interest \\ 
  85 & vacuum & tubes \\ 
  4253 & George & W. \\ 
   \hline
\end{tabular}
\caption{Word pairs that are lexical chunks following our definition (left neighbors).} 
\label{tab:word_pairs_left_lexical_chunks}
\end{table}


==> tables/jaccard_875/word_pairs_left_no_lexical_chunks.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 14:18:01 2023
\begin{table}[ht]
\centering
\begin{tabular}{rll}
  \hline
 & left\_word & word \\ 
  \hline
702 & The & Hybrid \\ 
  1353 & a & limited \\ 
  531 & from & this \\ 
  1361 & In & 2001 \\ 
  4167 & 2.0 & ) \\ 
  4678 & '' & , \\ 
  311 & water & routes \\ 
  2881 & 32 & on \\ 
  4132 & Burridge & ( \\ 
  1501 & had & joined \\ 
  4509 & is & also \\ 
  708 & , & often \\ 
  1066 & intended & to \\ 
  812 & former & species \\ 
  8164 & yielded & a \\ 
   \hline
\end{tabular}
\caption{Word pairs that are no lexical chunks following our definition (left neighbors).} 
\label{tab:word_pairs_left_no_lexical_chunks}
\end{table}


==> tables/jaccard_875/word_pairs_right_lexical_chunks.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 14:18:01 2023
\begin{table}[ht]
\centering
\begin{tabular}{rll}
  \hline
 & word & right\_word \\ 
  \hline
3919 & ice & hockey \\ 
  3433 & most & recent \\ 
  2453 & Air & Force \\ 
  118 & Sciurus & flammifer \\ 
  653 & women & 's \\ 
  146 & Miss & Universe \\ 
  252 & peer-reviewed & scientific \\ 
  4541 & Udo & Dirkschneider \\ 
  3699 & census-designated & place \\ 
  3161 & lead & single \\ 
  833 & home & games \\ 
  1195 & Italian & footballer \\ 
  3097 & Keshavarz & Sadr \\ 
  1984 & scientific & journal \\ 
  53 & professional & basketball \\ 
   \hline
\end{tabular}
\caption{Word pairs that are lexical chunks following our definition (right neighbors).} 
\label{tab:word_pairs_right_lexical_chunks}
\end{table}


==> tables/jaccard_875/word_pairs_right_no_lexical_chunks.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 14:18:02 2023
\begin{table}[ht]
\centering
\begin{tabular}{rll}
  \hline
 & word & right\_word \\ 
  \hline
738 & from & his \\ 
  678 & 2013 & Malwarebytes \\ 
  704 & available & through \\ 
  1349 & Radio & Times \\ 
  530 & 2nd & Runner-up \\ 
  1359 & pilot & of \\ 
  4277 & as & applied \\ 
  4870 & full & complexity \\ 
  310 & in & international \\ 
  2869 & 48 & BCE \\ 
  4182 & born & October \\ 
  1489 & designed & for \\ 
  4646 & by & Parlophone \\ 
  712 & body & of \\ 
  1064 & most & cited \\ 
   \hline
\end{tabular}
\caption{Word pairs that are no lexical chunks following our definition (right neighbors).} 
\label{tab:word_pairs_right_no_lexical_chunks}
\end{table}


==> tables/mi_like_875/importance_rating_model_anova_parametric.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 14:23:29 2023
\begin{table}[ht]
\centering
\begin{tabular}{rrrr}
  \hline
 & df & F & p-value \\ 
  \hline
capitalization & 2.00 & 3.23 & 0.04 \\ 
  dependency\_relation & 35.00 & 2.94 & 0.00 \\ 
   \hline
\end{tabular}
\caption{Parametric terms for $t=87.5\%$ and MI-like measure.} 
\label{tab:importance_rating_model_anova_parametric_mi_like_875}
\end{table}


==> tables/mi_like_875/importance_rating_model_anova_smooth.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 14:23:29 2023
\begin{table*}[ht]
\centering
\begin{tabular}{p{5cm}rrrr}
  \hline
 & edf & Ref.df & F & p-value \\ 
  \hline
s(saliency) & 11.21 & 19.00 & 584.57 & 0.00 \\ 
  s(display\_index) & 3.04 & 9.00 & 21.63 & 0.00 \\ 
  s(word\_length) & 1.63 & 9.00 & 16.66 & 0.00 \\ 
  s(sentence\_length) & 0.00 & 4.00 & 0.00 & 0.41 \\ 
  s(relative\_word\_frequency) & 0.00 & 9.00 & 0.00 & 0.81 \\ 
  s(normalized\_saliency\_rank) & 0.56 & 9.00 & 0.32 & 0.13 \\ 
  s(word\_position) & 0.65 & 9.00 & 0.22 & 0.16 \\ 
  te(left difference,saliency):\\no chunk & 3.10 & 24.00 & 1.57 & 0.00 \\ 
  te(left difference,saliency):\\chunk & 1.79 & 24.00 & 0.34 & 0.08 \\ 
  te(right difference,saliency):\\no chunk & 2.37 & 24.00 & 0.47 & 0.05 \\ 
  te(right difference,saliency):\\chunk & 0.64 & 24.00 & 0.05 & 0.25 \\ 
  s(sentence\_id) & 0.00 & 149.00 & 0.00 & 0.64 \\ 
  s(saliency,sentence\_id) & 17.14 & 150.00 & 0.15 & 0.16 \\ 
  s(worker\_id) & 62.19 & 63.00 & 30521.95 & 0.00 \\ 
  s(saliency,worker\_id) & 62.11 & 64.00 & 16749.25 & 0.00 \\ 
   \hline
\end{tabular}
\caption{Smooth terms for $t=87.5\%$ and MI-like measure.} \label{tab:importance_rating_model_anova_smooth_mi_like_875}
\end{table*}


==> tables/mi_like_875/importance_rating_model_params.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 14:23:41 2023
\begin{table}[ht]
\centering
\begin{tabular}{lrrrr}
   \hline
A. parametric coefficients & Estimate & Std. Error & t-value & p-value \\ 
  (Intercept) & 5.0206 & 0.5455 & 9.2030 & $<$ 0.0001 \\ 
  capitalizationall\_upper & 0.2472 & 0.1692 & 1.4613 & 0.1440 \\ 
  capitalizationfirst\_upper & 0.1501 & 0.0652 & 2.3026 & 0.0213 \\ 
  dependency\_relationacl & 0.6230 & 0.1710 & 3.6432 & 0.0003 \\ 
  dependency\_relationacl:relcl & 1.0768 & 0.2899 & 3.7142 & 0.0002 \\ 
  dependency\_relationadvcl & 0.9884 & 0.2166 & 4.5637 & $<$ 0.0001 \\ 
  dependency\_relationadvmod & 0.2472 & 0.1735 & 1.4246 & 0.1543 \\ 
  dependency\_relationamod & 0.6945 & 0.1298 & 5.3510 & $<$ 0.0001 \\ 
  dependency\_relationappos & 0.5602 & 0.1869 & 2.9966 & 0.0027 \\ 
  dependency\_relationaux & -0.0263 & 0.2510 & -0.1048 & 0.9165 \\ 
  dependency\_relationaux:pass & 0.4634 & 0.1677 & 2.7638 & 0.0057 \\ 
  dependency\_relationcase & 0.2977 & 0.0990 & 3.0061 & 0.0027 \\ 
  dependency\_relationcc & 0.0009 & 0.1738 & 0.0052 & 0.9959 \\ 
  dependency\_relationccomp & 0.4927 & 0.4680 & 1.0528 & 0.2925 \\ 
  dependency\_relationcompound & 0.6214 & 0.1239 & 5.0140 & $<$ 0.0001 \\ 
  dependency\_relationcompound:prt & 0.4353 & 0.5600 & 0.7773 & 0.4370 \\ 
  dependency\_relationconj & 0.5475 & 0.1678 & 3.2630 & 0.0011 \\ 
  dependency\_relationcop & 0.1856 & 0.1430 & 1.2984 & 0.1942 \\ 
  dependency\_relationdep & 1.3333 & 1.0652 & 1.2517 & 0.2107 \\ 
  dependency\_relationdet & 0.0742 & 0.1070 & 0.6932 & 0.4882 \\ 
  dependency\_relationdet:predet & 1.2635 & 0.7226 & 1.7484 & 0.0804 \\ 
  dependency\_relationfixed & -0.0353 & 0.4274 & -0.0827 & 0.9341 \\ 
  dependency\_relationflat & 0.6432 & 0.1500 & 4.2874 & $<$ 0.0001 \\ 
  dependency\_relationmark & 0.1152 & 0.2152 & 0.5354 & 0.5924 \\ 
  dependency\_relationnmod & 0.8162 & 0.1370 & 5.9598 & $<$ 0.0001 \\ 
  dependency\_relationnmod:poss & 0.6802 & 0.2110 & 3.2237 & 0.0013 \\ 
  dependency\_relationnmod:tmod & 0.7590 & 0.1740 & 4.3608 & $<$ 0.0001 \\ 
  dependency\_relationnsubj & 0.5009 & 0.1518 & 3.2998 & 0.0010 \\ 
  dependency\_relationnsubj:pass & 0.3896 & 0.2162 & 1.8019 & 0.0716 \\ 
  dependency\_relationnummod & 0.7870 & 0.2380 & 3.3070 & 0.0009 \\ 
  dependency\_relationobj & 0.6490 & 0.1515 & 4.2824 & $<$ 0.0001 \\ 
  dependency\_relationobl & 0.7723 & 0.1274 & 6.0625 & $<$ 0.0001 \\ 
  dependency\_relationobl:agent & 0.6005 & 0.3577 & 1.6790 & 0.0932 \\ 
  dependency\_relationobl:npmod & 0.3720 & 0.8048 & 0.4622 & 0.6440 \\ 
  dependency\_relationobl:tmod & 0.7757 & 0.2090 & 3.7123 & 0.0002 \\ 
  dependency\_relationparataxis & 0.9422 & 0.8511 & 1.1071 & 0.2683 \\ 
  dependency\_relationroot & 0.6849 & 0.1317 & 5.1993 & $<$ 0.0001 \\ 
  dependency\_relationxcomp & 0.6814 & 0.2658 & 2.5633 & 0.0104 \\ 
   \hline
B. smooth terms & edf & Ref.df & F-value & p-value \\ 
  s(saliency) & 11.2053 & 19.0000 & 584.5691 & $<$ 0.0001 \\ 
  s(display\_index) & 3.0407 & 9.0000 & 21.6345 & $<$ 0.0001 \\ 
  s(word\_length) & 1.6324 & 9.0000 & 16.6649 & $<$ 0.0001 \\ 
  s(sentence\_length) & 0.0005 & 4.0000 & 0.0001 & 0.4070 \\ 
  s(relative\_word\_frequency) & 0.0003 & 9.0000 & 0.0000 & 0.8135 \\ 
  s(normalized\_saliency\_rank) & 0.5572 & 9.0000 & 0.3165 & 0.1296 \\ 
  s(word\_position) & 0.6518 & 9.0000 & 0.2187 & 0.1590 \\ 
  te(left\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_leftFALSE & 3.0961 & 24.0000 & 1.5711 & 0.0010 \\ 
  te(left\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_leftTRUE & 1.7882 & 24.0000 & 0.3416 & 0.0824 \\ 
  te(right\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_rightFALSE & 2.3665 & 24.0000 & 0.4658 & 0.0476 \\ 
  te(right\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_rightTRUE & 0.6367 & 24.0000 & 0.0513 & 0.2489 \\ 
  s(sentence\_id) & 0.0018 & 149.0000 & 0.0000 & 0.6382 \\ 
  s(saliency,sentence\_id) & 17.1390 & 150.0000 & 0.1473 & 0.1646 \\ 
  s(worker\_id) & 62.1892 & 63.0000 & 30521.9491 & $<$ 0.0001 \\ 
  s(saliency,worker\_id) & 62.1082 & 64.0000 & 16749.2495 & $<$ 0.0001 \\ 
   \hline
\end{tabular}
\caption{Smooth and parametric terms.} 
\label{importance_rating_model_params}
\end{table}


==> tables/mi_like_875/word_pairs_left_lexical_chunks.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 14:21:38 2023
\begin{table}[ht]
\centering
\begin{tabular}{rll}
  \hline
 & left\_word & word \\ 
  \hline
958 & basketball & player \\ 
  568 & The & film \\ 
  157 & the & University \\ 
  6769 & World & Cup \\ 
  1716 & New & Zealand \\ 
  262 & UK & singles \\ 
  713 & This & article \\ 
  1495 & the & song \\ 
  4125 & an & English \\ 
  437 & the & second \\ 
  3320 & R & \& \\ 
  360 & Rock & band \\ 
  49 & the & city \\ 
  121 & an & American \\ 
  637 & a & small \\ 
   \hline
\end{tabular}
\caption{Word pairs that are lexical chunks following our definition (left neighbors).} 
\label{tab:word_pairs_left_lexical_chunks}
\end{table}


==> tables/mi_like_875/word_pairs_left_no_lexical_chunks.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 14:21:38 2023
\begin{table}[ht]
\centering
\begin{tabular}{rll}
  \hline
 & left\_word & word \\ 
  \hline
685 & Paweensuda & Drouin \\ 
  1327 & born & 18 \\ 
  515 & transport & are \\ 
  1337 & FC & Liefering \\ 
  3989 & der & Zijden \\ 
  4467 & range & of \\ 
  299 & synchronized & swimmer \\ 
  2766 & Athlyi & Rogers \\ 
  3922 & on & canvas \\ 
  1434 & selling & some \\ 
  4280 & has & been \\ 
  691 & into & a \\ 
  1028 & Conte & Professor \\ 
  800 & he & played \\ 
  7077 & in & critic \\ 
   \hline
\end{tabular}
\caption{Word pairs that are no lexical chunks following our definition (left neighbors).} 
\label{tab:word_pairs_left_no_lexical_chunks}
\end{table}


==> tables/mi_like_875/word_pairs_right_lexical_chunks.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 14:21:38 2023
\begin{table}[ht]
\centering
\begin{tabular}{rll}
  \hline
 & word & right\_word \\ 
  \hline
894 & south & Wales \\ 
  535 & a & number \\ 
  183 & an & Italian \\ 
  8386 & R & \& \\ 
  1750 & the & film \\ 
  226 & discus & throw \\ 
  655 & railway & station \\ 
  1505 & the & family \\ 
  4311 & Do & n't \\ 
  396 & the & U.S. \\ 
  2703 & football & team \\ 
  3839 & the & university \\ 
  263 & the & town \\ 
  23 & UK & singles \\ 
  58 & an & American \\ 
   \hline
\end{tabular}
\caption{Word pairs that are lexical chunks following our definition (right neighbors).} 
\label{tab:word_pairs_right_lexical_chunks}
\end{table}


==> tables/mi_like_875/word_pairs_right_no_lexical_chunks.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 14:21:39 2023
\begin{table}[ht]
\centering
\begin{tabular}{rll}
  \hline
 & word & right\_word \\ 
  \hline
712 & body & of \\ 
  654 & / & Psychology \\ 
  678 & 2013 & Malwarebytes \\ 
  1301 & classical & lyceum \\ 
  513 & best & finish \\ 
  1313 & protecting & water \\ 
  4073 & in & West \\ 
  4522 & oldest & , \\ 
  296 & classifications & . \\ 
  2715 & Baker & was \\ 
  4009 & retired & rally \\ 
  1417 & , & Malaysia \\ 
  4393 & Royal & Assent \\ 
  683 & was & also \\ 
  1013 & featuring & Udo \\ 
   \hline
\end{tabular}
\caption{Word pairs that are no lexical chunks following our definition (right neighbors).} 
\label{tab:word_pairs_right_no_lexical_chunks}
\end{table}


==> tables/phi_sq_25/importance_rating_model_anova_parametric.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 13:58:34 2023
\begin{table}[ht]
\centering
\begin{tabular}{rrrr}
  \hline
 & df & F & p-value \\ 
  \hline
capitalization & 2.00 & 3.01 & 0.05 \\ 
  dependency\_relation & 35.00 & 2.93 & 0.00 \\ 
   \hline
\end{tabular}
\caption{Parametric terms for $t=25\%$ and phi squared measure.} 
\label{tab:importance_rating_model_anova_parametric_phi_sq_25}
\end{table}


==> tables/phi_sq_25/importance_rating_model_anova_smooth.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 13:58:34 2023
\begin{table*}[ht]
\centering
\begin{tabular}{p{5cm}rrrr}
  \toprule
 & edf & Ref.df & F & p-value \\ 
  \midrule
s(saliency) & 11.23 & 19.00 & 547.16 & 0.00 \\ 
  s(display\_index) & 3.10 & 9.00 & 20.93 & 0.00 \\ 
  s(word\_length) & 1.61 & 9.00 & 16.47 & 0.00 \\ 
  s(sentence\_length) & 0.00 & 4.00 & 0.00 & 0.44 \\ 
  s(relative\_word\_frequency) & 0.00 & 9.00 & 0.00 & 0.81 \\ 
  s(normalized\_saliency\_rank) & 0.58 & 9.00 & 0.36 & 0.12 \\ 
  s(word\_position) & 0.59 & 9.00 & 0.18 & 0.17 \\ 
  te(left difference,saliency):\\no chunk & 2.90 & 24.00 & 1.21 & 0.00 \\ 
  te(left difference,saliency):\\chunk & 3.34 & 24.00 & 0.92 & 0.02 \\ 
  te(right difference,saliency):\\no chunk & 2.50 & 24.00 & 0.67 & 0.02 \\ 
  te(right difference,saliency):\\chunk & 0.00 & 24.00 & 0.00 & 0.84 \\ 
  s(sentence\_id) & 0.00 & 149.00 & 0.00 & 0.60 \\ 
  s(saliency,sentence\_id) & 17.35 & 150.00 & 0.15 & 0.18 \\ 
  s(worker\_id) & 62.19 & 63.00 & 30421.05 & 0.00 \\ 
  s(saliency,worker\_id) & 62.11 & 64.00 & 17591.01 & 0.00 \\ 
   \bottomrule
\end{tabular}
\caption{Smooth terms for $t=25\%$ and phi squared measure.} 
\label{tab:importance_rating_model_anova_smooth_phi_sq_25}
\end{table*}


==> tables/phi_sq_25/importance_rating_model_params.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 13:58:47 2023
\begin{table}[ht]
\centering
\begin{tabular}{lrrrr}
   \hline
A. parametric coefficients & Estimate & Std. Error & t-value & p-value \\ 
  (Intercept) & 5.0293 & 0.5455 & 9.2203 & $<$ 0.0001 \\ 
  capitalizationall\_upper & 0.2477 & 0.1691 & 1.4649 & 0.1430 \\ 
  capitalizationfirst\_upper & 0.1433 & 0.0653 & 2.1925 & 0.0284 \\ 
  dependency\_relationacl & 0.6210 & 0.1706 & 3.6402 & 0.0003 \\ 
  dependency\_relationacl:relcl & 1.0684 & 0.2895 & 3.6902 & 0.0002 \\ 
  dependency\_relationadvcl & 0.9896 & 0.2162 & 4.5774 & $<$ 0.0001 \\ 
  dependency\_relationadvmod & 0.2369 & 0.1731 & 1.3690 & 0.1710 \\ 
  dependency\_relationamod & 0.6559 & 0.1317 & 4.9782 & $<$ 0.0001 \\ 
  dependency\_relationappos & 0.5535 & 0.1872 & 2.9562 & 0.0031 \\ 
  dependency\_relationaux & -0.0171 & 0.2505 & -0.0683 & 0.9455 \\ 
  dependency\_relationaux:pass & 0.4642 & 0.1672 & 2.7755 & 0.0055 \\ 
  dependency\_relationcase & 0.2984 & 0.0988 & 3.0205 & 0.0025 \\ 
  dependency\_relationcc & -0.0128 & 0.1738 & -0.0739 & 0.9411 \\ 
  dependency\_relationccomp & 0.5124 & 0.4670 & 1.0974 & 0.2725 \\ 
  dependency\_relationcompound & 0.5842 & 0.1255 & 4.6541 & $<$ 0.0001 \\ 
  dependency\_relationcompound:prt & 0.4307 & 0.5597 & 0.7696 & 0.4416 \\ 
  dependency\_relationconj & 0.5327 & 0.1680 & 3.1705 & 0.0015 \\ 
  dependency\_relationcop & 0.1859 & 0.1427 & 1.3028 & 0.1927 \\ 
  dependency\_relationdep & 1.4256 & 1.0667 & 1.3364 & 0.1814 \\ 
  dependency\_relationdet & 0.0499 & 0.1078 & 0.4633 & 0.6432 \\ 
  dependency\_relationdet:predet & 1.2639 & 0.7201 & 1.7551 & 0.0793 \\ 
  dependency\_relationfixed & -0.0857 & 0.4252 & -0.2015 & 0.8403 \\ 
  dependency\_relationflat & 0.6314 & 0.1524 & 4.1417 & $<$ 0.0001 \\ 
  dependency\_relationmark & 0.1178 & 0.2146 & 0.5490 & 0.5831 \\ 
  dependency\_relationnmod & 0.8107 & 0.1371 & 5.9131 & $<$ 0.0001 \\ 
  dependency\_relationnmod:poss & 0.6381 & 0.2115 & 3.0173 & 0.0026 \\ 
  dependency\_relationnmod:tmod & 0.7594 & 0.1742 & 4.3583 & $<$ 0.0001 \\ 
  dependency\_relationnsubj & 0.5032 & 0.1522 & 3.3058 & 0.0010 \\ 
  dependency\_relationnsubj:pass & 0.3688 & 0.2176 & 1.6948 & 0.0901 \\ 
  dependency\_relationnummod & 0.7544 & 0.2383 & 3.1657 & 0.0016 \\ 
  dependency\_relationobj & 0.6518 & 0.1527 & 4.2697 & $<$ 0.0001 \\ 
  dependency\_relationobl & 0.7685 & 0.1278 & 6.0117 & $<$ 0.0001 \\ 
  dependency\_relationobl:agent & 0.5990 & 0.3591 & 1.6680 & 0.0953 \\ 
  dependency\_relationobl:npmod & 0.3855 & 0.8029 & 0.4801 & 0.6312 \\ 
  dependency\_relationobl:tmod & 0.7561 & 0.2097 & 3.6060 & 0.0003 \\ 
  dependency\_relationparataxis & 0.9426 & 0.8504 & 1.1083 & 0.2677 \\ 
  dependency\_relationroot & 0.6775 & 0.1315 & 5.1508 & $<$ 0.0001 \\ 
  dependency\_relationxcomp & 0.6667 & 0.2662 & 2.5046 & 0.0123 \\ 
   \hline
B. smooth terms & edf & Ref.df & F-value & p-value \\ 
  s(saliency) & 11.2261 & 19.0000 & 547.1555 & $<$ 0.0001 \\ 
  s(display\_index) & 3.1029 & 9.0000 & 20.9266 & $<$ 0.0001 \\ 
  s(word\_length) & 1.6103 & 9.0000 & 16.4682 & $<$ 0.0001 \\ 
  s(sentence\_length) & 0.0008 & 4.0000 & 0.0001 & 0.4355 \\ 
  s(relative\_word\_frequency) & 0.0004 & 9.0000 & 0.0000 & 0.8136 \\ 
  s(normalized\_saliency\_rank) & 0.5796 & 9.0000 & 0.3625 & 0.1202 \\ 
  s(word\_position) & 0.5870 & 9.0000 & 0.1814 & 0.1734 \\ 
  te(left\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_leftFALSE & 2.8991 & 24.0000 & 1.2062 & 0.0025 \\ 
  te(left\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_leftTRUE & 3.3435 & 24.0000 & 0.9173 & 0.0151 \\ 
  te(right\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_rightFALSE & 2.4969 & 24.0000 & 0.6683 & 0.0208 \\ 
  te(right\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_rightTRUE & 0.0009 & 24.0000 & 0.0000 & 0.8375 \\ 
  s(sentence\_id) & 0.0014 & 149.0000 & 0.0000 & 0.6014 \\ 
  s(saliency,sentence\_id) & 17.3458 & 150.0000 & 0.1483 & 0.1782 \\ 
  s(worker\_id) & 62.1877 & 63.0000 & 30421.0485 & $<$ 0.0001 \\ 
  s(saliency,worker\_id) & 62.1076 & 64.0000 & 17591.0087 & $<$ 0.0001 \\ 
   \hline
\end{tabular}
\caption{Smooth and parametric terms.} 
\label{importance_rating_model_params}
\end{table}


==> tables/phi_sq_25/word_pairs_left_lexical_chunks.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 13:56:41 2023
\begin{table}[ht]
\centering
\begin{tabular}{rll}
  \hline
 & left\_word & word \\ 
  \hline
2233 & a & rural \\ 
  2057 & retail & shops \\ 
  1254 & the & Cayman \\ 
  1714 & DeeJay & Gigolo \\ 
  834 & Mushroom & Records \\ 
  1950 & Electric & Indigo \\ 
  1360 & the & base \\ 
  9050 & limited & edition \\ 
  4345 & year-end & lists \\ 
  5990 & Charles & `` \\ 
  3226 & August & 1974 \\ 
  2853 & different & cover \\ 
  3066 & November & 1995 \\ 
  1813 & its & license \\ 
  4119 & Nastasia & Noens \\ 
   \hline
\end{tabular}
\caption{Word pairs that are lexical chunks following our definition (left neighbors).} 
\label{tab:word_pairs_left_lexical_chunks}
\end{table}


==> tables/phi_sq_25/word_pairs_left_no_lexical_chunks.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 13:56:41 2023
\begin{table}[ht]
\centering
\begin{tabular}{rll}
  \hline
 & left\_word & word \\ 
  \hline
475 & until & after \\ 
  8386 & features & R \\ 
  2678 & Merriam & Award \\ 
  1079 & Assent & on \\ 
  1772 & born & 8 \\ 
  1311 & to & knowledge \\ 
  2998 & T-71 & in \\ 
  276 & and & is \\ 
  92 & born & 1972 \\ 
  496 & station & licensed \\ 
  1932 & well & on \\ 
  2564 & were & also \\ 
  3638 & Marathon & , \\ 
  1000 & of & Hamburg \\ 
  925 & author & and \\ 
   \hline
\end{tabular}
\caption{Word pairs that are no lexical chunks following our definition (left neighbors).} 
\label{tab:word_pairs_left_no_lexical_chunks}
\end{table}


==> tables/phi_sq_25/word_pairs_right_lexical_chunks.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 13:56:41 2023
\begin{table}[ht]
\centering
\begin{tabular}{rll}
  \hline
 & word & right\_word \\ 
  \hline
2266 & an & American-Venezuelan \\ 
  2039 & landing & procedure \\ 
  1196 & of & `` \\ 
  1714 & Gigolo & Records \\ 
  842 & wildlife & stewardship \\ 
  1908 & Web & sites \\ 
  1353 & limited & quantity \\ 
  4923 & October & 6 \\ 
  7361 & the & title \\ 
  3433 & most & recent \\ 
  2836 & Fantography & submissions \\ 
  3169 & Salford & County \\ 
  1845 & FIVB & Volleyball \\ 
  4594 & similarly & themed \\ 
  7680 & known & thrombin \\ 
   \hline
\end{tabular}
\caption{Word pairs that are lexical chunks following our definition (right neighbors).} 
\label{tab:word_pairs_right_lexical_chunks}
\end{table}


==> tables/phi_sq_25/word_pairs_right_no_lexical_chunks.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 13:56:41 2023
\begin{table}[ht]
\centering
\begin{tabular}{rll}
  \hline
 & word & right\_word \\ 
  \hline
446 & by & International \\ 
  7050 & System & ( \\ 
  2578 & to & 1974 \\ 
  1059 & `` & nine \\ 
  1724 & Germany & , \\ 
  1274 & 's & victory \\ 
  2935 & ( & classical \\ 
  253 & ; & commission \\ 
  77 & 's & release \\ 
  464 & of & Being \\ 
  1843 & in & Dulecha \\ 
  2412 & craft & with \\ 
  3502 & takes & care \\ 
  977 & events & , \\ 
  904 & , & with \\ 
   \hline
\end{tabular}
\caption{Word pairs that are no lexical chunks following our definition (right neighbors).} 
\label{tab:word_pairs_right_no_lexical_chunks}
\end{table}


==> tables/phi_sq_50/importance_rating_model_anova_parametric.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 13:53:58 2023
\begin{table}[ht]
\centering
\begin{tabular}{rrrr}
  \hline
 & df & F & p-value \\ 
  \hline
capitalization & 2.00 & 2.95 & 0.05 \\ 
  dependency\_relation & 35.00 & 2.98 & 0.00 \\ 
   \hline
\end{tabular}
\caption{Parametric terms.} 
\label{importance_rating_model_anova_parametric}
\end{table}


==> tables/phi_sq_50/importance_rating_model_anova_smooth.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 13:53:58 2023
\begin{table}[ht]
\centering
\begin{tabular}{rrrrr}
  \hline
 & edf & Ref.df & F & p-value \\ 
  \hline
s(saliency) & 11.22 & 19.00 & 676.71 & 0.00 \\ 
  s(display\_index) & 3.09 & 9.00 & 21.85 & 0.00 \\ 
  s(word\_length) & 1.58 & 9.00 & 17.14 & 0.00 \\ 
  s(sentence\_length) & 0.00 & 4.00 & 0.00 & 0.38 \\ 
  s(relative\_word\_frequency) & 0.00 & 9.00 & 0.00 & 0.80 \\ 
  s(normalized\_saliency\_rank) & 0.57 & 9.00 & 0.34 & 0.12 \\ 
  s(word\_position) & 0.57 & 9.00 & 0.17 & 0.18 \\ 
  te(left\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_leftFALSE & 3.05 & 24.00 & 1.81 & 0.00 \\ 
  te(left\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_leftTRUE & 0.37 & 24.00 & 0.03 & 0.26 \\ 
  te(right\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_rightFALSE & 1.98 & 24.00 & 0.34 & 0.09 \\ 
  te(right\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_rightTRUE & 0.00 & 24.00 & 0.00 & 0.37 \\ 
  s(sentence\_id) & 0.00 & 149.00 & 0.00 & 0.33 \\ 
  s(saliency,sentence\_id) & 0.00 & 150.00 & 0.00 & 0.16 \\ 
  s(worker\_id) & 62.19 & 63.00 & 31510.84 & 0.00 \\ 
  s(saliency,worker\_id) & 62.11 & 64.00 & 17703.05 & 0.00 \\ 
   \hline
\end{tabular}
\caption{Smooth terms.} 
\label{importance_rating_model_anova_smooth}
\end{table}


==> tables/phi_sq_50/importance_rating_model_params.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 13:54:09 2023
\begin{table}[ht]
\centering
\begin{tabular}{lrrrr}
   \hline
A. parametric coefficients & Estimate & Std. Error & t-value & p-value \\ 
  (Intercept) & 5.0123 & 0.5443 & 9.2079 & $<$ 0.0001 \\ 
  capitalizationall\_upper & 0.2389 & 0.1681 & 1.4211 & 0.1553 \\ 
  capitalizationfirst\_upper & 0.1413 & 0.0648 & 2.1826 & 0.0291 \\ 
  dependency\_relationacl & 0.6265 & 0.1701 & 3.6839 & 0.0002 \\ 
  dependency\_relationacl:relcl & 1.0790 & 0.2889 & 3.7353 & 0.0002 \\ 
  dependency\_relationadvcl & 1.0022 & 0.2151 & 4.6591 & $<$ 0.0001 \\ 
  dependency\_relationadvmod & 0.2361 & 0.1722 & 1.3713 & 0.1703 \\ 
  dependency\_relationamod & 0.6786 & 0.1296 & 5.2362 & $<$ 0.0001 \\ 
  dependency\_relationappos & 0.5685 & 0.1857 & 3.0610 & 0.0022 \\ 
  dependency\_relationaux & -0.0087 & 0.2497 & -0.0349 & 0.9722 \\ 
  dependency\_relationaux:pass & 0.4603 & 0.1666 & 2.7625 & 0.0057 \\ 
  dependency\_relationcase & 0.2976 & 0.0983 & 3.0277 & 0.0025 \\ 
  dependency\_relationcc & -0.0025 & 0.1728 & -0.0142 & 0.9886 \\ 
  dependency\_relationccomp & 0.4894 & 0.4651 & 1.0523 & 0.2927 \\ 
  dependency\_relationcompound & 0.6101 & 0.1235 & 4.9396 & $<$ 0.0001 \\ 
  dependency\_relationcompound:prt & 0.4207 & 0.5572 & 0.7550 & 0.4502 \\ 
  dependency\_relationconj & 0.5483 & 0.1666 & 3.2912 & 0.0010 \\ 
  dependency\_relationcop & 0.1815 & 0.1425 & 1.2738 & 0.2028 \\ 
  dependency\_relationdep & 1.3826 & 1.0673 & 1.2955 & 0.1952 \\ 
  dependency\_relationdet & 0.0660 & 0.1066 & 0.6190 & 0.5359 \\ 
  dependency\_relationdet:predet & 1.2392 & 0.7170 & 1.7282 & 0.0840 \\ 
  dependency\_relationfixed & -0.0898 & 0.4228 & -0.2124 & 0.8318 \\ 
  dependency\_relationflat & 0.6539 & 0.1496 & 4.3717 & $<$ 0.0001 \\ 
  dependency\_relationmark & 0.1236 & 0.2137 & 0.5782 & 0.5631 \\ 
  dependency\_relationnmod & 0.8208 & 0.1359 & 6.0404 & $<$ 0.0001 \\ 
  dependency\_relationnmod:poss & 0.6642 & 0.2097 & 3.1676 & 0.0015 \\ 
  dependency\_relationnmod:tmod & 0.7638 & 0.1735 & 4.4019 & $<$ 0.0001 \\ 
  dependency\_relationnsubj & 0.4993 & 0.1510 & 3.3053 & 0.0010 \\ 
  dependency\_relationnsubj:pass & 0.3768 & 0.2152 & 1.7507 & 0.0800 \\ 
  dependency\_relationnummod & 0.7657 & 0.2367 & 3.2352 & 0.0012 \\ 
  dependency\_relationobj & 0.6570 & 0.1509 & 4.3526 & $<$ 0.0001 \\ 
  dependency\_relationobl & 0.7662 & 0.1266 & 6.0510 & $<$ 0.0001 \\ 
  dependency\_relationobl:agent & 0.6029 & 0.3564 & 1.6920 & 0.0907 \\ 
  dependency\_relationobl:npmod & 0.3617 & 0.8033 & 0.4503 & 0.6525 \\ 
  dependency\_relationobl:tmod & 0.7617 & 0.2091 & 3.6428 & 0.0003 \\ 
  dependency\_relationparataxis & 0.9627 & 0.8473 & 1.1362 & 0.2559 \\ 
  dependency\_relationroot & 0.6860 & 0.1308 & 5.2447 & $<$ 0.0001 \\ 
  dependency\_relationxcomp & 0.6961 & 0.2648 & 2.6289 & 0.0086 \\ 
   \hline
B. smooth terms & edf & Ref.df & F-value & p-value \\ 
  s(saliency) & 11.2215 & 19.0000 & 676.7094 & $<$ 0.0001 \\ 
  s(display\_index) & 3.0906 & 9.0000 & 21.8508 & $<$ 0.0001 \\ 
  s(word\_length) & 1.5814 & 9.0000 & 17.1385 & $<$ 0.0001 \\ 
  s(sentence\_length) & 0.0005 & 4.0000 & 0.0001 & 0.3815 \\ 
  s(relative\_word\_frequency) & 0.0004 & 9.0000 & 0.0000 & 0.8039 \\ 
  s(normalized\_saliency\_rank) & 0.5701 & 9.0000 & 0.3417 & 0.1246 \\ 
  s(word\_position) & 0.5726 & 9.0000 & 0.1742 & 0.1788 \\ 
  te(left\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_leftFALSE & 3.0524 & 24.0000 & 1.8115 & 0.0004 \\ 
  te(left\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_leftTRUE & 0.3726 & 24.0000 & 0.0258 & 0.2615 \\ 
  te(right\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_rightFALSE & 1.9798 & 24.0000 & 0.3413 & 0.0891 \\ 
  te(right\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_rightTRUE & 0.0013 & 24.0000 & 0.0001 & 0.3660 \\ 
  s(sentence\_id) & 0.0017 & 149.0000 & 0.0000 & 0.3284 \\ 
  s(saliency,sentence\_id) & 0.0019 & 150.0000 & 0.0000 & 0.1572 \\ 
  s(worker\_id) & 62.1873 & 63.0000 & 31510.8427 & $<$ 0.0001 \\ 
  s(saliency,worker\_id) & 62.1059 & 64.0000 & 17703.0545 & $<$ 0.0001 \\ 
   \hline
\end{tabular}
\caption{Smooth and parametric terms.} 
\label{importance_rating_model_params}
\end{table}


==> tables/phi_sq_50/word_pairs_left_lexical_chunks.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 13:52:06 2023
\begin{table}[ht]
\centering
\begin{tabular}{rll}
  \hline
 & left\_word & word \\ 
  \hline
3113 & April & 7 \\ 
  7055 & older & brother \\ 
  1274 & Caesar & 's \\ 
  1921 & and & producer \\ 
  4738 & Saeed & Soltani \\ 
  3973 & St & Mirren \\ 
  2072 & technology & company \\ 
  3273 & The & original \\ 
  7168 & women & 's \\ 
  1315 & original & version \\ 
  3790 & February & 2010 \\ 
  2316 & racing & cyclist \\ 
  1147 & Minor & Counties \\ 
  367 & English & cricketer \\ 
  6149 & All & My \\ 
   \hline
\end{tabular}
\caption{Word pairs that are lexical chunks following our definition (left neighbors).} 
\label{tab:word_pairs_left_lexical_chunks}
\end{table}


==> tables/phi_sq_50/word_pairs_left_no_lexical_chunks.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 13:52:06 2023
\begin{table}[ht]
\centering
\begin{tabular}{rll}
  \hline
 & left\_word & word \\ 
  \hline
1339 & named & after \\ 
  955 & general & runners \\ 
  865 & for & Outstanding \\ 
  894 & , & south \\ 
  1856 & Chiodo & also \\ 
  681 & retired & rally \\ 
  1873 & 2012 & via \\ 
  407 & publish & the \\ 
  4492 & born & September \\ 
  2061 & Allen & Larue \\ 
  904 & 1979 & , \\ 
  1435 & still & be \\ 
  1068 & Fargo & , \\ 
  2317 & film & Valentine \\ 
  251 & FIFA & announced \\ 
   \hline
\end{tabular}
\caption{Word pairs that are no lexical chunks following our definition (left neighbors).} 
\label{tab:word_pairs_left_no_lexical_chunks}
\end{table}


==> tables/phi_sq_50/word_pairs_right_lexical_chunks.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 13:52:06 2023
\begin{table}[ht]
\centering
\begin{tabular}{rll}
  \hline
 & word & right\_word \\ 
  \hline
3335 & June & 2011 \\ 
  9214 & New & Orleans \\ 
  1197 & an & elliptical \\ 
  1845 & FIVB & Volleyball \\ 
  5089 & a & long-time \\ 
  4393 & Royal & Assent \\ 
  1984 & scientific & journal \\ 
  3436 & Caesar & 's \\ 
  1268 & a & Dutch \\ 
  4102 & professional & golfer \\ 
  2365 & IRIB & TV3 \\ 
  1038 & February & 2017 \\ 
  389 & Computer & Science \\ 
  7218 & compilation & album \\ 
  657 & Music/Theater & Projects \\ 
   \hline
\end{tabular}
\caption{Word pairs that are lexical chunks following our definition (right neighbors).} 
\label{tab:word_pairs_right_lexical_chunks}
\end{table}


==> tables/phi_sq_50/word_pairs_right_no_lexical_chunks.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 13:52:06 2023
\begin{table}[ht]
\centering
\begin{tabular}{rll}
  \hline
 & word & right\_word \\ 
  \hline
945 & Lavery & on \\ 
  869 & Hinnant & ( \\ 
  902 & 18 & , \\ 
  1800 & and & is \\ 
  692 & eighteen & districts \\ 
  1824 & ( & soccer \\ 
  392 & Electric & Indigo \\ 
  4417 & has & explained \\ 
  2018 & president & ) \\ 
  908 & event & at \\ 
  1415 & painting & by \\ 
  1059 & `` & nine \\ 
  2253 & enabling & Phase \\ 
  232 & 's & first \\ 
  69 & , & PAR3 \\ 
   \hline
\end{tabular}
\caption{Word pairs that are no lexical chunks following our definition (right neighbors).} 
\label{tab:word_pairs_right_no_lexical_chunks}
\end{table}


==> tables/phi_sq_75/importance_rating_model_anova_parametric.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 13:38:12 2023
\begin{table}[ht]
\centering
\begin{tabular}{rrrr}
  \hline
 & df & F & p-value \\ 
  \hline
capitalization & 2.00 & 3.01 & 0.05 \\ 
  dependency\_relation & 35.00 & 2.96 & 0.00 \\ 
   \hline
\end{tabular}
\caption{Parametric terms.} 
\label{importance_rating_model_anova_parametric}
\end{table}


==> tables/phi_sq_75/importance_rating_model_anova_smooth.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 13:38:12 2023
\begin{table}[ht]
\centering
\begin{tabular}{rrrrr}
  \hline
 & edf & Ref.df & F & p-value \\ 
  \hline
s(saliency) & 11.22 & 19.00 & 608.07 & 0.00 \\ 
  s(display\_index) & 3.03 & 9.00 & 21.56 & 0.00 \\ 
  s(word\_length) & 1.61 & 9.00 & 16.76 & 0.00 \\ 
  s(sentence\_length) & 0.00 & 4.00 & 0.00 & 0.42 \\ 
  s(relative\_word\_frequency) & 0.00 & 9.00 & 0.00 & 0.79 \\ 
  s(normalized\_saliency\_rank) & 0.55 & 9.00 & 0.29 & 0.13 \\ 
  s(word\_position) & 0.62 & 9.00 & 0.20 & 0.17 \\ 
  te(left\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_leftFALSE & 3.10 & 24.00 & 1.50 & 0.00 \\ 
  te(left\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_leftTRUE & 1.64 & 24.00 & 0.30 & 0.09 \\ 
  te(right\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_rightFALSE & 2.88 & 24.00 & 0.82 & 0.01 \\ 
  te(right\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_rightTRUE & 0.00 & 24.00 & 0.00 & 0.83 \\ 
  s(sentence\_id) & 0.00 & 149.00 & 0.00 & 0.32 \\ 
  s(saliency,sentence\_id) & 0.00 & 150.00 & 0.00 & 0.15 \\ 
  s(worker\_id) & 62.19 & 63.00 & 29859.19 & 0.00 \\ 
  s(saliency,worker\_id) & 62.11 & 64.00 & 17411.36 & 0.00 \\ 
   \hline
\end{tabular}
\caption{Smooth terms.} 
\label{importance_rating_model_anova_smooth}
\end{table}


==> tables/phi_sq_75/importance_rating_model_params.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 13:38:24 2023
\begin{table}[ht]
\centering
\begin{tabular}{lrrrr}
   \hline
A. parametric coefficients & Estimate & Std. Error & t-value & p-value \\ 
  (Intercept) & 5.0415 & 0.5449 & 9.2518 & $<$ 0.0001 \\ 
  capitalizationall\_upper & 0.2394 & 0.1683 & 1.4224 & 0.1549 \\ 
  capitalizationfirst\_upper & 0.1431 & 0.0647 & 2.2103 & 0.0271 \\ 
  dependency\_relationacl & 0.6223 & 0.1704 & 3.6513 & 0.0003 \\ 
  dependency\_relationacl:relcl & 1.0774 & 0.2889 & 3.7293 & 0.0002 \\ 
  dependency\_relationadvcl & 0.9924 & 0.2155 & 4.6050 & $<$ 0.0001 \\ 
  dependency\_relationadvmod & 0.2372 & 0.1726 & 1.3743 & 0.1694 \\ 
  dependency\_relationamod & 0.6804 & 0.1294 & 5.2582 & $<$ 0.0001 \\ 
  dependency\_relationappos & 0.5604 & 0.1861 & 3.0107 & 0.0026 \\ 
  dependency\_relationaux & -0.0154 & 0.2498 & -0.0616 & 0.9509 \\ 
  dependency\_relationaux:pass & 0.4580 & 0.1669 & 2.7445 & 0.0061 \\ 
  dependency\_relationcase & 0.2945 & 0.0985 & 2.9908 & 0.0028 \\ 
  dependency\_relationcc & 0.0025 & 0.1731 & 0.0142 & 0.9887 \\ 
  dependency\_relationccomp & 0.4856 & 0.4655 & 1.0432 & 0.2969 \\ 
  dependency\_relationcompound & 0.6086 & 0.1234 & 4.9306 & $<$ 0.0001 \\ 
  dependency\_relationcompound:prt & 0.4126 & 0.5574 & 0.7403 & 0.4591 \\ 
  dependency\_relationconj & 0.5420 & 0.1669 & 3.2465 & 0.0012 \\ 
  dependency\_relationcop & 0.1769 & 0.1426 & 1.2404 & 0.2148 \\ 
  dependency\_relationdep & 1.3494 & 1.0636 & 1.2687 & 0.2046 \\ 
  dependency\_relationdet & 0.0658 & 0.1065 & 0.6183 & 0.5364 \\ 
  dependency\_relationdet:predet & 1.2301 & 0.7184 & 1.7123 & 0.0869 \\ 
  dependency\_relationfixed & -0.0733 & 0.4237 & -0.1729 & 0.8627 \\ 
  dependency\_relationflat & 0.6494 & 0.1496 & 4.3414 & $<$ 0.0001 \\ 
  dependency\_relationmark & 0.1162 & 0.2140 & 0.5429 & 0.5872 \\ 
  dependency\_relationnmod & 0.8162 & 0.1362 & 5.9942 & $<$ 0.0001 \\ 
  dependency\_relationnmod:poss & 0.6711 & 0.2099 & 3.1978 & 0.0014 \\ 
  dependency\_relationnmod:tmod & 0.7590 & 0.1734 & 4.3760 & $<$ 0.0001 \\ 
  dependency\_relationnsubj & 0.4973 & 0.1513 & 3.2876 & 0.0010 \\ 
  dependency\_relationnsubj:pass & 0.3772 & 0.2152 & 1.7525 & 0.0797 \\ 
  dependency\_relationnummod & 0.7724 & 0.2368 & 3.2616 & 0.0011 \\ 
  dependency\_relationobj & 0.6534 & 0.1510 & 4.3271 & $<$ 0.0001 \\ 
  dependency\_relationobl & 0.7659 & 0.1268 & 6.0400 & $<$ 0.0001 \\ 
  dependency\_relationobl:agent & 0.5895 & 0.3563 & 1.6544 & 0.0981 \\ 
  dependency\_relationobl:npmod & 0.3636 & 0.8033 & 0.4526 & 0.6508 \\ 
  dependency\_relationobl:tmod & 0.7576 & 0.2089 & 3.6268 & 0.0003 \\ 
  dependency\_relationparataxis & 0.9443 & 0.8470 & 1.1148 & 0.2650 \\ 
  dependency\_relationroot & 0.6829 & 0.1312 & 5.2035 & $<$ 0.0001 \\ 
  dependency\_relationxcomp & 0.6870 & 0.2649 & 2.5933 & 0.0095 \\ 
   \hline
B. smooth terms & edf & Ref.df & F-value & p-value \\ 
  s(saliency) & 11.2185 & 19.0000 & 608.0696 & $<$ 0.0001 \\ 
  s(display\_index) & 3.0290 & 9.0000 & 21.5602 & $<$ 0.0001 \\ 
  s(word\_length) & 1.6145 & 9.0000 & 16.7580 & $<$ 0.0001 \\ 
  s(sentence\_length) & 0.0009 & 4.0000 & 0.0002 & 0.4181 \\ 
  s(relative\_word\_frequency) & 0.0004 & 9.0000 & 0.0000 & 0.7891 \\ 
  s(normalized\_saliency\_rank) & 0.5463 & 9.0000 & 0.2930 & 0.1346 \\ 
  s(word\_position) & 0.6177 & 9.0000 & 0.1974 & 0.1676 \\ 
  te(left\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_leftFALSE & 3.0957 & 24.0000 & 1.5001 & 0.0015 \\ 
  te(left\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_leftTRUE & 1.6363 & 24.0000 & 0.3020 & 0.0874 \\ 
  te(right\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_rightFALSE & 2.8765 & 24.0000 & 0.8205 & 0.0145 \\ 
  te(right\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_rightTRUE & 0.0009 & 24.0000 & 0.0000 & 0.8279 \\ 
  s(sentence\_id) & 0.0015 & 149.0000 & 0.0000 & 0.3231 \\ 
  s(saliency,sentence\_id) & 0.0016 & 150.0000 & 0.0000 & 0.1459 \\ 
  s(worker\_id) & 62.1882 & 63.0000 & 29859.1932 & $<$ 0.0001 \\ 
  s(saliency,worker\_id) & 62.1070 & 64.0000 & 17411.3567 & $<$ 0.0001 \\ 
   \hline
\end{tabular}
\caption{Smooth and parametric terms.} 
\label{importance_rating_model_params}
\end{table}


==> tables/phi_sq_75/word_pairs_left_lexical_chunks.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 13:36:18 2023
\begin{table}[ht]
\centering
\begin{tabular}{rll}
  \hline
 & left\_word & word \\ 
  \hline
1172 & universal & acclaim \\ 
  5986 & a & German \\ 
  4804 & elliptical & galaxy \\ 
  27 & the & title \\ 
  3112 & freight & forwarding \\ 
  2268 & lead & single \\ 
  149 & W. & Bush \\ 
  1263 & All-Ireland & medal \\ 
  6157 & second & single \\ 
  5340 & Udo & Dirkschneider \\ 
  1984 & peer-reviewed & scientific \\ 
  367 & English & cricketer \\ 
  3655 & Federal & Communications \\ 
  948 & Special & Scientific \\ 
  4253 & George & W. \\ 
   \hline
\end{tabular}
\caption{Word pairs that are lexical chunks following our definition (left neighbors).} 
\label{tab:word_pairs_left_lexical_chunks}
\end{table}


==> tables/phi_sq_75/word_pairs_left_no_lexical_chunks.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 13:36:19 2023
\begin{table}[ht]
\centering
\begin{tabular}{rll}
  \hline
 & left\_word & word \\ 
  \hline
1075 & later & playing \\ 
  800 & he & played \\ 
  728 & After & completion \\ 
  756 & son & Frank \\ 
  1503 & theory & and \\ 
  576 & of & George \\ 
  1513 & for & Year \\ 
  5137 & based & out \\ 
  6005 & the & 2009 \\ 
  341 & to & develop \\ 
  3220 & available & through \\ 
  5055 & Philip & Wight \\ 
  1633 & several & area \\ 
  5675 & are & three \\ 
  761 & teachers/students & teaching/studying \\ 
   \hline
\end{tabular}
\caption{Word pairs that are no lexical chunks following our definition (left neighbors).} 
\label{tab:word_pairs_left_no_lexical_chunks}
\end{table}


==> tables/phi_sq_75/word_pairs_right_lexical_chunks.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 13:36:19 2023
\begin{table}[ht]
\centering
\begin{tabular}{rll}
  \hline
 & word & right\_word \\ 
  \hline
894 & south & Wales \\ 
  4581 & the & new \\ 
  4250 & Major & League \\ 
  58 & an & American \\ 
  2741 & radio & station \\ 
  1870 & the & second \\ 
  208 & soap & operas \\ 
  1038 & February & 2017 \\ 
  4597 & Rajesh & Khanna \\ 
  4399 & North & Dakota \\ 
  1650 & Kana & Kanmani \\ 
  394 & All-Ireland & medal \\ 
  3464 & Patria & Music/Theater \\ 
  755 & American & professional \\ 
  3922 & canvas & painting \\ 
   \hline
\end{tabular}
\caption{Word pairs that are lexical chunks following our definition (right neighbors).} 
\label{tab:word_pairs_right_lexical_chunks}
\end{table}


==> tables/phi_sq_75/word_pairs_right_no_lexical_chunks.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 13:36:19 2023
\begin{table}[ht]
\centering
\begin{tabular}{rll}
  \hline
 & word & right\_word \\ 
  \hline
1077 & Harry & Fisher \\ 
  808 & Regency & as \\ 
  733 & role & of \\ 
  764 & substrates & metabolized \\ 
  1507 & Samuel & D. \\ 
  567 & England & and \\ 
  1515 & singer & Ciara \\ 
  5278 & Wetumpka & , \\ 
  6240 & Psychology & . \\ 
  326 & filming & was \\ 
  3271 & platform & to \\ 
  5169 & Kalckhoff & ( \\ 
  1648 & be & classified \\ 
  5901 & were & produced \\ 
  777 & , & highly \\ 
   \hline
\end{tabular}
\caption{Word pairs that are no lexical chunks following our definition (right neighbors).} 
\label{tab:word_pairs_right_no_lexical_chunks}
\end{table}


==> tables/phi_sq_875/importance_rating_model_anova_parametric.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 13:24:50 2023
\begin{table}[ht]
\centering
\begin{tabular}{rrrr}
  \hline
 & df & F & p-value \\ 
  \hline
capitalization & 2.00 & 3.15 & \textbf{0.042} \\ 
  dependency relation & 35.00 & 2.92 & \textbf{$<$ 0.0001} \\ 
   \hline
\end{tabular}
\caption{Wald tests for the parametric terms (using $t=87.5\%$ and phi squared measure). TODO: Use standrad p ranges..} 
\label{tab:importance_rating_model_anova_parametric_phi_sq_875}
\end{table}


==> tables/phi_sq_875/importance_rating_model_anova_smooth.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 13:24:50 2023
\begin{table*}[ht]
\centering

\resizebox{0.77\linewidth}{!}{
\begin{tabular}{p{6cm}rrrr}
  \toprule
 & edf & Ref.df & F & p-value \\ 
  \midrule
  s(saliency) & 11.22 & 19.00 & 580.89 & \textbf{$<$ 0.0001} \\ 
  s(display index) & 3.04 & 9.00 & 22.02 & \textbf{$<$ 0.0001} \\ 
  s(word length) & 1.64 & 9.00 & 16.44 & \textbf{$<$ 0.0001} \\ 
  s(sentence length) & 0.00 & 4.00 & 0.00 & 0.425 \\ 
  s(relative word frequency) & 0.00 & 9.00 & 0.00 & 0.844 \\ 
  s(normalized saliency rank) & 0.59 & 9.00 & 0.37 & 0.115 \\ 
  s(word position) & 0.58 & 9.00 & 0.18 & 0.177 \\ 
  te(left difference,saliency): no chunk & 3.12 & 24.00 & 1.50 & \textbf{0.002} \\ 
  te(left difference,saliency): chunk & 2.24 & 24.00 & 0.51 & \textbf{0.0038} \\ 
  te(right difference,saliency): no chunk & 2.43 & 24.00 & 0.47 & \textbf{0.049} \\ 
  te(right difference,saliency): chunk & 0.00 & 24.00 & 0.00 & 0.578 \\ 
  s(sentence ID) & 0.00 & 149.00 & 0.00 & 0.616 \\ 
  s(saliency,sentence ID) & 16.13 & 150.00 & 0.14 & 0.191 \\ 
  s(worker ID) & 62.19 & 63.00 & 30911.89 & \textbf{$<$ 0.0001} \\ 
  s(saliency,worker ID) & 62.11 & 64.00 & 16760.88 & \textbf{$<$ 0.0001} \\ 
   \bottomrule
\end{tabular} }
\caption{Effective degrees of freedom (edf), reference df and Wald test statistics for the univariate smooth terms (using $t=87.5\%$ and phi squared measure).} 
\label{tab:importance_rating_model_anova_smooth_phi_sq_875}
\end{table*}


==> tables/phi_sq_875/importance_rating_model_params.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 13:25:02 2023
\begin{table}[ht]
\centering
\begin{tabular}{lrrrr}
   \hline
A. parametric coefficients & Estimate & Std. Error & t-value & p-value \\ 
  (Intercept) & 5.0312 & 0.5457 & 9.2196 & $<$ 0.0001 \\ 
  capitalizationall\_upper & 0.2454 & 0.1692 & 1.4502 & 0.1470 \\ 
  capitalizationfirst\_upper & 0.1479 & 0.0652 & 2.2689 & 0.0233 \\ 
  dependency\_relationacl & 0.6199 & 0.1710 & 3.6257 & 0.0003 \\ 
  dependency\_relationacl:relcl & 1.0729 & 0.2898 & 3.7026 & 0.0002 \\ 
  dependency\_relationadvcl & 0.9863 & 0.2165 & 4.5558 & $<$ 0.0001 \\ 
  dependency\_relationadvmod & 0.2433 & 0.1734 & 1.4028 & 0.1607 \\ 
  dependency\_relationamod & 0.6897 & 0.1298 & 5.3147 & $<$ 0.0001 \\ 
  dependency\_relationappos & 0.5576 & 0.1870 & 2.9826 & 0.0029 \\ 
  dependency\_relationaux & -0.0275 & 0.2508 & -0.1097 & 0.9127 \\ 
  dependency\_relationaux:pass & 0.4598 & 0.1676 & 2.7437 & 0.0061 \\ 
  dependency\_relationcase & 0.2970 & 0.0990 & 3.0002 & 0.0027 \\ 
  dependency\_relationcc & 0.0007 & 0.1738 & 0.0040 & 0.9968 \\ 
  dependency\_relationccomp & 0.4931 & 0.4679 & 1.0539 & 0.2920 \\ 
  dependency\_relationcompound & 0.6156 & 0.1239 & 4.9669 & $<$ 0.0001 \\ 
  dependency\_relationcompound:prt & 0.4317 & 0.5599 & 0.7710 & 0.4407 \\ 
  dependency\_relationconj & 0.5427 & 0.1678 & 3.2351 & 0.0012 \\ 
  dependency\_relationcop & 0.1828 & 0.1430 & 1.2790 & 0.2009 \\ 
  dependency\_relationdep & 1.3371 & 1.0657 & 1.2546 & 0.2096 \\ 
  dependency\_relationdet & 0.0776 & 0.1066 & 0.7276 & 0.4669 \\ 
  dependency\_relationdet:predet & 1.2669 & 0.7227 & 1.7528 & 0.0797 \\ 
  dependency\_relationfixed & -0.0416 & 0.4265 & -0.0975 & 0.9223 \\ 
  dependency\_relationflat & 0.6438 & 0.1501 & 4.2882 & $<$ 0.0001 \\ 
  dependency\_relationmark & 0.1132 & 0.2151 & 0.5261 & 0.5988 \\ 
  dependency\_relationnmod & 0.8150 & 0.1369 & 5.9516 & $<$ 0.0001 \\ 
  dependency\_relationnmod:poss & 0.6845 & 0.2107 & 3.2485 & 0.0012 \\ 
  dependency\_relationnmod:tmod & 0.7565 & 0.1740 & 4.3467 & $<$ 0.0001 \\ 
  dependency\_relationnsubj & 0.4932 & 0.1518 & 3.2483 & 0.0012 \\ 
  dependency\_relationnsubj:pass & 0.3851 & 0.2160 & 1.7830 & 0.0746 \\ 
  dependency\_relationnummod & 0.7837 & 0.2379 & 3.2938 & 0.0010 \\ 
  dependency\_relationobj & 0.6425 & 0.1515 & 4.2397 & $<$ 0.0001 \\ 
  dependency\_relationobl & 0.7688 & 0.1274 & 6.0358 & $<$ 0.0001 \\ 
  dependency\_relationobl:agent & 0.5944 & 0.3575 & 1.6625 & 0.0964 \\ 
  dependency\_relationobl:npmod & 0.3674 & 0.8046 & 0.4565 & 0.6480 \\ 
  dependency\_relationobl:tmod & 0.7755 & 0.2089 & 3.7132 & 0.0002 \\ 
  dependency\_relationparataxis & 0.9400 & 0.8507 & 1.1049 & 0.2692 \\ 
  dependency\_relationroot & 0.6789 & 0.1317 & 5.1530 & $<$ 0.0001 \\ 
  dependency\_relationxcomp & 0.6800 & 0.2658 & 2.5583 & 0.0105 \\ 
   \hline
B. smooth terms & edf & Ref.df & F-value & p-value \\ 
  s(saliency) & 11.2191 & 19.0000 & 580.8899 & $<$ 0.0001 \\ 
  s(display\_index) & 3.0359 & 9.0000 & 22.0213 & $<$ 0.0001 \\ 
  s(word\_length) & 1.6357 & 9.0000 & 16.4381 & $<$ 0.0001 \\ 
  s(sentence\_length) & 0.0005 & 4.0000 & 0.0001 & 0.4252 \\ 
  s(relative\_word\_frequency) & 0.0003 & 9.0000 & 0.0000 & 0.8444 \\ 
  s(normalized\_saliency\_rank) & 0.5905 & 9.0000 & 0.3662 & 0.1151 \\ 
  s(word\_position) & 0.5843 & 9.0000 & 0.1772 & 0.1771 \\ 
  te(left\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_leftFALSE & 3.1217 & 24.0000 & 1.5032 & 0.0020 \\ 
  te(left\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_leftTRUE & 2.2358 & 24.0000 & 0.5119 & 0.0383 \\ 
  te(right\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_rightFALSE & 2.4313 & 24.0000 & 0.4734 & 0.0491 \\ 
  te(right\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_rightTRUE & 0.0016 & 24.0000 & 0.0001 & 0.5778 \\ 
  s(sentence\_id) & 0.0015 & 149.0000 & 0.0000 & 0.6160 \\ 
  s(saliency,sentence\_id) & 16.1258 & 150.0000 & 0.1363 & 0.1908 \\ 
  s(worker\_id) & 62.1895 & 63.0000 & 30911.8893 & $<$ 0.0001 \\ 
  s(saliency,worker\_id) & 62.1083 & 64.0000 & 16760.8772 & $<$ 0.0001 \\ 
   \hline
\end{tabular}
\caption{Smooth and parametric terms.} 
\label{importance_rating_model_params}
\end{table}


==> tables/phi_sq_875/word_pairs_left_lexical_chunks.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 13:22:55 2023
\begin{table}[ht]
\centering
\begin{tabular}{rll}
  \hline
 & left\_word & word \\ 
  \hline
4253 & George & W. \\ 
  3819 & most & recent \\ 
  3129 & box & office \\ 
  149 & W. & Bush \\ 
  896 & railway & station \\ 
  171 & Triple & J \\ 
  304 & fairy & tale \\ 
  6448 & Malayalam & film \\ 
  4021 & the & United \\ 
  3521 & United & Kingdom \\ 
  1195 & an & Italian \\ 
  1724 & Nazi & Germany \\ 
  3436 & Julius & Caesar \\ 
  2606 & Major & League \\ 
  114 & a & species \\ 
   \hline
\end{tabular}
\caption{Word pairs that are lexical chunks following our definition (left neighbors).} 
\label{tab:word_pairs_left_lexical_chunks}
\end{table}


==> tables/phi_sq_875/word_pairs_left_no_lexical_chunks.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 13:22:55 2023
\begin{table}[ht]
\centering
\begin{tabular}{rll}
  \hline
 & left\_word & word \\ 
  \hline
735 & , & including \\ 
  678 & December & 2013 \\ 
  705 & Outstanding & Public \\ 
  1355 & Andrew & Viterbi \\ 
  531 & from & this \\ 
  1364 & for & minor-league \\ 
  4189 & procedure & . \\ 
  4782 & Malwarebytes & announced \\ 
  311 & water & routes \\ 
  2886 & 1993 & , \\ 
  4141 & a & software \\ 
  1498 & preceded & by \\ 
  4549 & 1889 & oil \\ 
  711 & The & black-throated \\ 
  1069 & home & to \\ 
   \hline
\end{tabular}
\caption{Word pairs that are no lexical chunks following our definition (left neighbors).} 
\label{tab:word_pairs_left_no_lexical_chunks}
\end{table}


==> tables/phi_sq_875/word_pairs_right_lexical_chunks.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 13:22:56 2023
\begin{table}[ht]
\centering
\begin{tabular}{rll}
  \hline
 & word & right\_word \\ 
  \hline
3919 & ice & hockey \\ 
  3464 & Patria & Music/Theater \\ 
  2703 & football & team \\ 
  142 & feature & films \\ 
  744 & as & well \\ 
  155 & backing & vocals \\ 
  351 & City & Council \\ 
  4399 & North & Dakota \\ 
  3699 & census-designated & place \\ 
  3307 & Aulacorhynchus & atrogularis \\ 
  948 & Scientific & Interest \\ 
  1424 & Federal & Communications \\ 
  3161 & lead & single \\ 
  2212 & Beaux & Arts \\ 
  58 & an & American \\ 
   \hline
\end{tabular}
\caption{Word pairs that are lexical chunks following our definition (right neighbors).} 
\label{tab:word_pairs_right_lexical_chunks}
\end{table}


==> tables/phi_sq_875/word_pairs_right_no_lexical_chunks.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 13:22:56 2023
\begin{table}[ht]
\centering
\begin{tabular}{rll}
  \hline
 & word & right\_word \\ 
  \hline
728 & completion & of \\ 
  670 & of & Hamburg \\ 
  696 & of & Cedar \\ 
  1345 & and & philosophy \\ 
  526 & was & released \\ 
  1352 & into & law \\ 
  4275 & in & this \\ 
  4875 & to & this \\ 
  306 & documentaries & . \\ 
  2863 & public & and \\ 
  4176 & then-President & George \\ 
  1480 & 2012 & via \\ 
  4653 & officially & launched \\ 
  704 & available & through \\ 
  1049 & born & February \\ 
   \hline
\end{tabular}
\caption{Word pairs that are no lexical chunks following our definition (right neighbors).} 
\label{tab:word_pairs_right_no_lexical_chunks}
\end{table}


==> tables/poisson_stirling_875/importance_rating_model_anova_parametric.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 14:16:32 2023
\begin{table}[ht]
\centering
\begin{tabular}{rrrr}
  \hline
 & df & F & p-value \\ 
  \hline
capitalization & 2.00 & 3.19 & 0.04 \\ 
  dependency\_relation & 35.00 & 2.95 & 0.00 \\ 
   \hline
\end{tabular}
\caption{Parametric terms.} 
\label{importance_rating_model_anova_parametric}
\end{table}


==> tables/poisson_stirling_875/importance_rating_model_anova_smooth.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 14:16:32 2023
\begin{table}[ht]
\centering
\begin{tabular}{rrrrr}
  \hline
 & edf & Ref.df & F & p-value \\ 
  \hline
s(saliency) & 11.21 & 19.00 & 585.59 & 0.00 \\ 
  s(display\_index) & 3.04 & 9.00 & 21.73 & 0.00 \\ 
  s(word\_length) & 1.62 & 9.00 & 16.48 & 0.00 \\ 
  s(sentence\_length) & 0.00 & 4.00 & 0.00 & 0.39 \\ 
  s(relative\_word\_frequency) & 0.00 & 9.00 & 0.00 & 0.84 \\ 
  s(normalized\_saliency\_rank) & 0.55 & 9.00 & 0.31 & 0.13 \\ 
  s(word\_position) & 0.66 & 9.00 & 0.22 & 0.16 \\ 
  te(left\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_leftFALSE & 3.15 & 24.00 & 1.69 & 0.00 \\ 
  te(left\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_leftTRUE & 1.20 & 24.00 & 0.17 & 0.13 \\ 
  te(right\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_rightFALSE & 2.27 & 24.00 & 0.44 & 0.05 \\ 
  te(right\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_rightTRUE & 0.53 & 24.00 & 0.05 & 0.22 \\ 
  s(sentence\_id) & 0.00 & 149.00 & 0.00 & 0.64 \\ 
  s(saliency,sentence\_id) & 16.96 & 150.00 & 0.15 & 0.17 \\ 
  s(worker\_id) & 62.19 & 63.00 & 30367.39 & 0.00 \\ 
  s(saliency,worker\_id) & 62.11 & 64.00 & 16940.52 & 0.00 \\ 
   \hline
\end{tabular}
\caption{Smooth terms.} 
\label{importance_rating_model_anova_smooth}
\end{table}


==> tables/poisson_stirling_875/importance_rating_model_params.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 14:16:44 2023
\begin{table}[ht]
\centering
\begin{tabular}{lrrrr}
   \hline
A. parametric coefficients & Estimate & Std. Error & t-value & p-value \\ 
  (Intercept) & 5.0203 & 0.5455 & 9.2028 & $<$ 0.0001 \\ 
  capitalizationall\_upper & 0.2482 & 0.1692 & 1.4672 & 0.1424 \\ 
  capitalizationfirst\_upper & 0.1486 & 0.0652 & 2.2797 & 0.0226 \\ 
  dependency\_relationacl & 0.6244 & 0.1709 & 3.6543 & 0.0003 \\ 
  dependency\_relationacl:relcl & 1.0779 & 0.2898 & 3.7192 & 0.0002 \\ 
  dependency\_relationadvcl & 0.9900 & 0.2164 & 4.5741 & $<$ 0.0001 \\ 
  dependency\_relationadvmod & 0.2485 & 0.1733 & 1.4340 & 0.1516 \\ 
  dependency\_relationamod & 0.6951 & 0.1296 & 5.3640 & $<$ 0.0001 \\ 
  dependency\_relationappos & 0.5624 & 0.1868 & 3.0106 & 0.0026 \\ 
  dependency\_relationaux & -0.0247 & 0.2509 & -0.0985 & 0.9216 \\ 
  dependency\_relationaux:pass & 0.4643 & 0.1676 & 2.7706 & 0.0056 \\ 
  dependency\_relationcase & 0.2986 & 0.0989 & 3.0174 & 0.0026 \\ 
  dependency\_relationcc & 0.0021 & 0.1738 & 0.0122 & 0.9903 \\ 
  dependency\_relationccomp & 0.4952 & 0.4679 & 1.0583 & 0.2899 \\ 
  dependency\_relationcompound & 0.6246 & 0.1237 & 5.0507 & $<$ 0.0001 \\ 
  dependency\_relationcompound:prt & 0.4357 & 0.5601 & 0.7779 & 0.4366 \\ 
  dependency\_relationconj & 0.5486 & 0.1676 & 3.2728 & 0.0011 \\ 
  dependency\_relationcop & 0.1865 & 0.1429 & 1.3049 & 0.1919 \\ 
  dependency\_relationdep & 1.3350 & 1.0654 & 1.2530 & 0.2102 \\ 
  dependency\_relationdet & 0.0765 & 0.1069 & 0.7161 & 0.4739 \\ 
  dependency\_relationdet:predet & 1.2631 & 0.7223 & 1.7488 & 0.0804 \\ 
  dependency\_relationfixed & -0.0428 & 0.4260 & -0.1006 & 0.9199 \\ 
  dependency\_relationflat & 0.6471 & 0.1499 & 4.3177 & $<$ 0.0001 \\ 
  dependency\_relationmark & 0.1159 & 0.2151 & 0.5387 & 0.5901 \\ 
  dependency\_relationnmod & 0.8175 & 0.1368 & 5.9776 & $<$ 0.0001 \\ 
  dependency\_relationnmod:poss & 0.6815 & 0.2108 & 3.2325 & 0.0012 \\ 
  dependency\_relationnmod:tmod & 0.7604 & 0.1739 & 4.3725 & $<$ 0.0001 \\ 
  dependency\_relationnsubj & 0.5019 & 0.1516 & 3.3094 & 0.0009 \\ 
  dependency\_relationnsubj:pass & 0.3921 & 0.2161 & 1.8140 & 0.0697 \\ 
  dependency\_relationnummod & 0.7882 & 0.2379 & 3.3130 & 0.0009 \\ 
  dependency\_relationobj & 0.6503 & 0.1514 & 4.2955 & $<$ 0.0001 \\ 
  dependency\_relationobl & 0.7736 & 0.1272 & 6.0811 & $<$ 0.0001 \\ 
  dependency\_relationobl:agent & 0.6026 & 0.3576 & 1.6850 & 0.0920 \\ 
  dependency\_relationobl:npmod & 0.3762 & 0.8047 & 0.4675 & 0.6401 \\ 
  dependency\_relationobl:tmod & 0.7760 & 0.2090 & 3.7139 & 0.0002 \\ 
  dependency\_relationparataxis & 0.9441 & 0.8511 & 1.1092 & 0.2674 \\ 
  dependency\_relationroot & 0.6862 & 0.1315 & 5.2173 & $<$ 0.0001 \\ 
  dependency\_relationxcomp & 0.6834 & 0.2657 & 2.5719 & 0.0101 \\ 
   \hline
B. smooth terms & edf & Ref.df & F-value & p-value \\ 
  s(saliency) & 11.2093 & 19.0000 & 585.5920 & $<$ 0.0001 \\ 
  s(display\_index) & 3.0376 & 9.0000 & 21.7331 & $<$ 0.0001 \\ 
  s(word\_length) & 1.6151 & 9.0000 & 16.4800 & $<$ 0.0001 \\ 
  s(sentence\_length) & 0.0009 & 4.0000 & 0.0002 & 0.3944 \\ 
  s(relative\_word\_frequency) & 0.0005 & 9.0000 & 0.0000 & 0.8386 \\ 
  s(normalized\_saliency\_rank) & 0.5542 & 9.0000 & 0.3106 & 0.1308 \\ 
  s(word\_position) & 0.6562 & 9.0000 & 0.2205 & 0.1592 \\ 
  te(left\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_leftFALSE & 3.1513 & 24.0000 & 1.6946 & 0.0006 \\ 
  te(left\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_leftTRUE & 1.1998 & 24.0000 & 0.1733 & 0.1264 \\ 
  te(right\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_rightFALSE & 2.2699 & 24.0000 & 0.4405 & 0.0511 \\ 
  te(right\_neighbor\_saliency\_difference,saliency):cooccurrence\_and\_constituent\_rightTRUE & 0.5283 & 24.0000 & 0.0475 & 0.2167 \\ 
  s(sentence\_id) & 0.0010 & 149.0000 & 0.0000 & 0.6357 \\ 
  s(saliency,sentence\_id) & 16.9584 & 150.0000 & 0.1452 & 0.1713 \\ 
  s(worker\_id) & 62.1892 & 63.0000 & 30367.3907 & $<$ 0.0001 \\ 
  s(saliency,worker\_id) & 62.1080 & 64.0000 & 16940.5196 & $<$ 0.0001 \\ 
   \hline
\end{tabular}
\caption{Smooth and parametric terms.} 
\label{importance_rating_model_params}
\end{table}


==> tables/poisson_stirling_875/word_pairs_left_lexical_chunks.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 14:14:38 2023
\begin{table}[ht]
\centering
\begin{tabular}{rll}
  \hline
 & left\_word & word \\ 
  \hline
896 & railway & station \\ 
  568 & The & film \\ 
  150 & radio & station \\ 
  6769 & World & Cup \\ 
  1833 & the & university \\ 
  241 & the & film \\ 
  713 & This & article \\ 
  1629 & census-designated & place \\ 
  4125 & an & English \\ 
  437 & the & second \\ 
  3349 & south & Wales \\ 
  360 & Rock & band \\ 
  23 & the & UK \\ 
  114 & a & species \\ 
  637 & a & small \\ 
   \hline
\end{tabular}
\caption{Word pairs that are lexical chunks following our definition (left neighbors).} 
\label{tab:word_pairs_left_lexical_chunks}
\end{table}


==> tables/poisson_stirling_875/word_pairs_left_no_lexical_chunks.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 14:14:38 2023
\begin{table}[ht]
\centering
\begin{tabular}{rll}
  \hline
 & left\_word & word \\ 
  \hline
685 & Paweensuda & Drouin \\ 
  1327 & born & 18 \\ 
  515 & transport & are \\ 
  1337 & FC & Liefering \\ 
  3975 & Hanseatic & Trade \\ 
  4454 & for & students \\ 
  299 & synchronized & swimmer \\ 
  2755 & , & Reggie \\ 
  3919 & American & ice \\ 
  1433 & following & on \\ 
  4275 & succeeded & in \\ 
  691 & into & a \\ 
  1031 & for & protease-activated \\ 
  801 & made & to \\ 
  7055 & older & brother \\ 
   \hline
\end{tabular}
\caption{Word pairs that are no lexical chunks following our definition (left neighbors).} 
\label{tab:word_pairs_left_no_lexical_chunks}
\end{table}


==> tables/poisson_stirling_875/word_pairs_right_lexical_chunks.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 14:14:38 2023
\begin{table}[ht]
\centering
\begin{tabular}{rll}
  \hline
 & word & right\_word \\ 
  \hline
1055 & basketball & player \\ 
  744 & as & well \\ 
  262 & singles & chart \\ 
  7218 & compilation & album \\ 
  2398 & a & species \\ 
  396 & the & U.S. \\ 
  894 & south & Wales \\ 
  1882 & the & UK \\ 
  4021 & United & Kingdom \\ 
  653 & women & 's \\ 
  535 & a & number \\ 
  58 & an & American \\ 
  183 & an & Italian \\ 
  765 & a & retired \\ 
  5850 & the & last \\ 
   \hline
\end{tabular}
\caption{Word pairs that are lexical chunks following our definition (right neighbors).} 
\label{tab:word_pairs_right_lexical_chunks}
\end{table}


==> tables/poisson_stirling_875/word_pairs_right_no_lexical_chunks.tex <==
% latex table generated in R 4.0.3 by xtable 1.8-4 package
% Tue Jan 10 14:14:38 2023
\begin{table}[ht]
\centering
\begin{tabular}{rll}
  \hline
 & word & right\_word \\ 
  \hline
1292 & and & census-designated \\ 
  507 & women & that \\ 
  1302 & is & considered \\ 
  4009 & retired & rally \\ 
  4466 & born & John \\ 
  292 & located & on \\ 
  2690 & and & twice \\ 
  3963 & frontman & Jimmy \\ 
  1407 & album & also \\ 
  4311 & Do & n't \\ 
  678 & 2013 & Malwarebytes \\ 
  1005 & ORCi & ) \\ 
  786 & well & on \\ 
  6883 & custom & house \\ 
  4280 & been & named \\ 
   \hline
\end{tabular}
\caption{Word pairs that are no lexical chunks following our definition (right neighbors).} 
\label{tab:word_pairs_right_no_lexical_chunks}
\end{table}

